Cygnus A jointly calibrated and imaged via non-convex optimisation from VLA data

Radio interferometric (RI) data are noisy under-sampled spatial Fourier components of the unknown radio sky affected by direction-dependent antenna gains. Failure to model these antenna gains accurately results in a radio sky estimate with limited fidelity and resolution. The RI inverse problem has been recently addressed via a joint calibration and imaging approach which consists in solving a non-convex minimisation task, involving suitable priors for the DDEs, namely temporal and spatial smoothness, and sparsity for the unknown radio map via an $\ell_1$-norm prior, in the context of realistic RI simulations. Building on these developments, we propose to promote sparsity of the radio map via a log-sum prior, enforcing sparsity more strongly than the $\ell_1$-norm. The resulting minimisation task is addressed via a sequence of non-convex minimisation tasks composed of re-weighted $\ell_1$ image priors, which are solved approximately. We demonstrate the efficiency of the approach on RI observations of the celebrated radio galaxy Cygnus~A obtained with the Karl G. Jansky Very Large Array at X, C, and S bands. More precisely, we showcase that the approach enhances data fidelity significantly while achieving high resolution high dynamic range radio maps, confirming the suitability of the priors considered for the unknown DDEs and radio image. As a clear qualitative indication of the high fidelity achieved by the data and the proposed approach, we report the detection of three background sources in the vicinity of Cyg~A, at S band.

==> srcfiles/fig_xband_ddes_image_full.tex <==
\begin{figure*}
\begin{minipage}[t]{1\linewidth}
\centering
\includegraphics[width=0.27\linewidth]{figs/X/DDES/x_dde-A-1_l-5e-07_ant-1__full.jpg}
\includegraphics[width=0.26\linewidth]{figs/X/DDES/x_dde-A-1_l-1e-07_ant-1__full.jpg}
\includegraphics[width=0.26\linewidth]{/X/DDES/x_dde-A-1_sara_ant-1__full.jpg}
\includegraphics[width=0.27\linewidth]{/X/DDES/x_dde-A-1_l-5e-07_ant-26__full.jpg}
\includegraphics[width=0.26\linewidth]{/X/DDES/x_dde-A-1_l-1e-07_ant-26__full.jpg}
\includegraphics[width=0.26\linewidth]{/X/DDES/x_dde-A-1_sara_ant-26__full.jpg}
\end{minipage}
~\\
\begin{minipage}[t]{1\linewidth}
\centering
\includegraphics[width=0.27\linewidth]{/X/DDES/x_dde-A-2_l-5e-07_ant-1__full.jpg}
\includegraphics[width=0.26\linewidth]{/X/DDES/x_dde-A-2_l-1e-07_ant-1__full.jpg}
\includegraphics[width=0.26\linewidth]{/X/DDES/x_dde-A-2_sara_ant-1__full.jpg}
\includegraphics[width=0.27\linewidth]{/X/DDES/x_dde-A-2_l-5e-07_ant-27__full.jpg}
\includegraphics[width=0.26\linewidth]{/X/DDES/x_dde-A-2_l-1e-07_ant-27__full.jpg}
\includegraphics[width=0.26\linewidth]{/X/DDES/x_dde-A-2_sara_ant-27__full.jpg}
\end{minipage}
~\\
\begin{minipage}[t]{1\linewidth}\centering
\includegraphics[width=0.27\linewidth]{/X/DDES/x_dde-B_l-5e-07_ant-1__full.jpg}
\includegraphics[width=0.26\linewidth]{/X/DDES/x_dde-B_l-1e-07_ant-1__full.jpg}
\includegraphics[width=0.26\linewidth]{/X/DDES/x_dde-B_sara_ant-1__full.jpg}
\includegraphics[width=0.27\linewidth]{/X/DDES/x_dde-B_l-5e-07_ant-26__full.jpg}
\includegraphics[width=0.26\linewidth]{/X/DDES/x_dde-B_l-1e-07_ant-26__full.jpg}
\includegraphics[width=0.26\linewidth]{/X/DDES/x_dde-B_sara_ant-26__full.jpg}
\end{minipage}
~\\
\begin{minipage}[t]{1\linewidth}\centering
\includegraphics[width=0.27\linewidth]{/X/DDES/x_dde-C_l-5e-07_ant-1__full.jpg}
\includegraphics[width=0.26\linewidth]{/X/DDES/x_dde-C_l-1e-07_ant-1__full.jpg}
\includegraphics[width=0.26\linewidth]{/X/DDES/x_dde-C_sara_ant-1__full.jpg}
\includegraphics[width=0.27\linewidth]{/X/DDES/x_dde-C_l-5e-07_ant-26__full.jpg}
\includegraphics[width=0.26\linewidth]{/X/DDES/x_dde-C_l-1e-07_ant-26__full.jpg}
\includegraphics[width=0.26\linewidth]{/X/DDES/x_dde-C_sara_ant-26__full.jpg}
\end{minipage}
~\\
\begin{minipage}[t]{1\linewidth}\centering
\includegraphics[width=0.27\linewidth]{/X/DDES/x_dde-D_l-5e-07_ant-1__full.jpg}
\includegraphics[width=0.26\linewidth]{/X/DDES/x_dde-D_l-1e-07_ant-1__full.jpg}
\includegraphics[width=0.26\linewidth]{/X/DDES/x_dde-D_sara_ant-1__full.jpg}
\includegraphics[width=0.27\linewidth]{/X/DDES/x_dde-D_l-5e-07_ant-25__full.jpg}
\includegraphics[width=0.26\linewidth]{/X/DDES/x_dde-D_l-1e-07_ant-25__full.jpg}
\includegraphics[width=0.26\linewidth]{/X/DDES/x_dde-D_sara_ant-25__full.jpg}
\end{minipage}
\caption{X band: amplitudes of DDE solutions in the image domain obtained with our approach ($S=5\times 5,~\tau =8$). Estimated DDEs are displayed at pixel positions spanning six orders of magnitude of the recovered dynamic range in the image estimate. From left to right, results obtained with {the $\ell_1$ prior associated with regularisation} parameters $\check{\eta}=5\times 10^{-7}$ and $\check{\eta}= 10^{-7}$, respectively, and SARA prior with regularisation parameter $\check{\eta}=5 \times10^{-7}$. From top to bottom, DDE estimates of two chosen antennas for each of the VLA configurations at our {{chosen time slot}}. Rows 1-2, configuration A, first data set, antennas 1 and 26.  Rows 3-4, configuration A, second data set, antennas 1 and 27. Rows 5-6, configuration B, antennas 1 and 26. Rows 7-8, configuration C, antennas 1 and 26. Rows 9-10, configuration D, antennas 1 and 26. }
\label{fig:x_dde_solutions_full}
\end{figure*}

